Seek for Success: A Visualization Approach for Understanding the Dynamics of Academic Careers

How to achieve academic career success has been a long-standing research question in social science research. With the growing availability of large-scale well-documented academic profiles and career trajectories, scholarly interest in career success has been reinvigorated, which has emerged to be an active research domain called the Science of Science (i.e., SciSci). In this study, we adopt an innovative dynamic perspective to examine how individual and social factors will influence career success over time. We propose ACSeeker, an interactive visual analytics approach to explore the potential factors of success and how the influence of multiple factors changes at different stages of academic careers. We first applied a Multi-factor Impact Analysis framework to estimate the effect of different factors on academic career success over time. We then developed a visual analytics system to understand the dynamic effects interactively. A novel timeline is designed to reveal and compare the factor impacts based on the whole population. A customized career line showing the individual career development is provided to allow a detailed inspection. To validate the effectiveness and usability of ACSeeker, we report two case studies and interviews with a social scientist and general researchers.

==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/00_Abstract_history/00_Abstract_20210320.tex <==
\abstract{
How to achieve academic career success has become an active topic in multiple fields such as the science of science (i.e., SciSci) and career mobility, with the growing availability of \wyf{academic profiles} such as publications and researcher careers. 
\wyf{It can reflect the scientific production of researchers and further facilitate the development of the research community.} 
In this study, we work on the visualization community as an example to study how different factors affect academic career success over a long period. 
However, existing works in both SciSci and career mobility are inadequate to study academic careers, given multi-factors including social relations with a long time. 
Most of them focus on a single factor and the statistical methods are either tailored at static analysis or require significant efforts. 
We propose \textit{\systemname}, an interactive visual analytics approach to study \textbf{A}cademic \textbf{C}areer \textbf{S}uccess with multiple factors from a dynamic perspective. 
We first applied an enhanced sequence-history-analysis-based framework to estimate the impacts of different factors on academic career success over time. 
We then developed a visual analytics system to explore the dynamic effects on academic career success interactively. 
A novel timeline is designed to reveal the dynamic impacts of different factors over the whole research population. 
A customized career line showing the individual career development is provided to allow a detailed inspection. 
To validate the effectiveness and usability of \textit{\systemname}, we report two case studies and an interview with experts in sociology. 
} % end of abstract

==> sections/00_Abstract_history/00_Abstract_20210321_v1.tex <==
\abstract{
How to achieve academic career success has been a long-standing research question in social science research. 
With the growing availability of large-scale well-documented academic profiles and career trajectories, scholarly interest in career success has been reinvigorated which has emerged to be an active research domain called the science of science (i.e., SciSci). 
% \wyf{However, most existing works focus on the impact analysis of a single factor on career success. 
% They either adopt static approaches or require significant efforts.} 
In this study, we adopt an innovative dynamic perspective to examine how individual and social factors will influence career success over time. 
We propose \textit{\systemname}, an interactive visual analytics approach to understand \textbf{A}cademic \textbf{C}areer \textbf{S}uccess, 
% which takes into account the impacts of multiple factors from a dynamic perspective. 
which takes into account the impact evolvement of multiple factors. 
We first applied an enhanced sequence-history-analysis-based framework to estimate the impacts of different factors on academic career success over time. 
We then developed a visual analytics system to assist in exploring the dynamic effects on career success interactively. 
A novel timeline is designed to reveal and compare the factor impacts based on the whole population. 
A customized career line showing the individual career development is provided to allow a detailed inspection. 
To validate the effectiveness and usability of \textit{\systemname}, we report two case studies and an interview with experts in sociology.
} 

==> sections/01_Introduction_history/01_Introduction_20210228.tex <==
\firstsection{Introduction}
\label{sec:01_Introduction}
\maketitle
% 1. concept: career mobility. and its importance
How do you land a job and how to obtain career success? 
Nowadays, career mobility has been widely studied in multiple disciplines such as sociology and computer science. 
It studies career paths and the factors influencing them. 
It is essential to understand social mobility and inequality at the macro population level and facilitate job hunting and human resource planning at the micro individual level. 

% 2. concept: social network affecting career mobility/success
% 2-1 以前的career data analysis虽然是动态的分析，但是缺少network
These disciplines mostly regard career paths as \wyf{``independent linear chains of events''}. 
They aim to find common trajectory patterns or predict upcoming career events using sequence analysis. 
However, networking may also play an important role to achieve career success in specific circumstances according to social network researchers~\cite{shipilov2014network}. 
The sharing of resources among the social network such as knowledge may influence the career development. 
% that individuals' career paths have mutual effects in specific circumstances. 
This leads to a line of studies in sociology to explore how different social networks (i.e., social capital) can affect ones' career success~\cite{seibert2001social, adler2002social, shipilov2014network}. 
For example, within an organization, institutional relationships such as mentorships might lead to ones' faster promotion due to a quick improving of the knowledge and expertise when working with mentors~\cite{smith2000diversity, zacher2019academic}. 
Another example is academic careers, different collaborations of researchers may also have an impact on their scientific performances. 

% 2-2 以前也有工作分析social capital + career mobility, 但是缺少dynamic视角
However, these current attempts analyze the effect of networking on career success using simple statistic methods based on static networks obtained at the present time.
They are limited to study the problem in a static manner, while ignoring the dynamic change of individuals' networks, let alone analyzing the dynamic effects of networking on their career success evolvement. 
Moreover, the current statistic-based methods require significant efforts for analysis. 
They are ill-suited for the efficient exploration of career mobility with networking from overview to details, thus hindering sociologists from understanding the findings detected due to large amount of data. 
These obstacles have motivated us to utilize visual analytics to analyze career mobility and networking affect dynamically and interactively. 
However, developing such a visual analytics system faces three challenges.

% 3. Three challenges for developing a visualization system
% 3-1 model
First, extracting career mobility patterns and analyzing the networking effects are difficult. 
Identifying typical career patterns for a set of trajectories is difficult given the diverse lengths of career paths. 
The effects of networking on career development can vary along different time periods. 
Thus, a sophisticated model is required to distill prototypical mobility patterns and further analyze the networking affects on individuals' career success. 
% 3-2 visualization design
Second, depicting career mobility with networking effect is challenging. 
Given a large set of individual career paths, the visual representations of these sequences would suffer a great scalability problem, let along revealing social networks and their effects on these career paths. 
% 3-3 visual analytics system
Third, supporting interactive exploration of the career mobility from overview to details with comparison and reasoning is non-trivial. 
Apart from typical career patterns of groups, sociologists also desiderate to explore the career data in different levels of detail (LODs) to understand the result in a more comprehensive approach~\cite{shneiderman2003eyes}. 
An interactive visualization system with additional statistics for further reasoning is thus required. 

% 4-our methods
To address above challenges, we first proposed a novel framework based on sequence history analysis (i.e., SHA)~\cite{rossignon2018sequence} to detect the career mobility patterns along with the network effects by combining career mobility data with dynamic social network data. 
We then propose a novel visual design to reveal career mobility patterns from different levels of detail, with social networks embedded. 
\wyf{To be added with visual encoding details.}
Based on the framework and visual design, we further propose \textit{\systemname}, an interactive visualization system that assists sociologists in exploring career mobility, analyzing networking effects, and comparing and reasoning diverse mobility patterns at different periods. 
Our contributions are listed as follows: 
\vspace{-0.2cm}
\begin{itemize}
    \item We proposed a novel SHA-based framework that extract career mobility patterns and analyze networking effects on one's career success at different time periods. 
    \vspace{-0.2cm}
    \item We design and develop \textit{\systemname}, an interactive visualization system that enables sociologists to identify and explore insightful patterns of career mobility with networking with a novel sequence+network design. 
    % We propose a novel design which embeds social networks into the career sequences to facilitate mobility exploration. 
    \vspace{-0.2cm}
    \item \wyf{We demonstrate the effectiveness and usability of \textit{\systemname} with a real world usage scenario.} 
\end{itemize}



 


==> sections/01_Introduction_history/01_Introduction_20210317.tex <==
\firstsection{Introduction}
\label{sec:01_Introduction}
\maketitle
% 1. concept: career mobility. and its importance
Nowadays, career mobility has been widely studied in both sociology and data science, which studies career paths and the factors influencing them. 
It is essential to understand social mobility at the population level and facilitate career success (e.g., job level and income) at the individual level. 

% 2. academic career success
As a unique scenario, academic careers has attracted the attention of multiple groups including \wyf{sociologists and general researchers}. 
Sociologists focus on how different factors influence career success, which is a major topic in life-course data analysis. 
General researchers are concerned with questions like how to raise scientific productions and achieve their academic career success. 
These have brought a heated discussion in the area of Science of science (i.e., SciSci)~\cite{fortunato2018science}. 
Researchers use the academy profiles such as publications and citations to understand how different factors that may drive academic career success. 
It can further facilitate decision-making and raise scientific production of the whole research community. 
% 3. 然而现在的工作都不是特别够
% 3-1 SciSci - 很多工作（VIS领域的几个paper）：只注重一个角度的分析or只是多角度泛泛而谈。不分析多因素影响career success + 动态分析, based on a specific population
However, most of the SciSci works hold a single focus (e.g., collaboration~\cite{li2019early} or gender disparities~\cite{huang2020historical}) to analyze the academic success. 
Hardly have them traced a specific group of researchers longitudinally to compare the multi-factor impact on the career success along time. 
This could be essential to understand the problem from a dynamic perspective and also reflect the evolution of a specific field. 

% 3-2 以前的career data analysis虽然是动态的分析，但是缺少network
Career mobility studies have considered the career developments from a temporal perspective. 
They aim to find common trajectories or predict upcoming career events using sequence analysis. 
Nevertheless, social relations such as collaboration may also play an important role in achieving career success~\cite{li2019early, shipilov2014network}. 
The sharing of resources such as knowledge through social relations may also influence the academic career success. 
% 3-3 以前也有工作分析social capital + career mobility, 但是缺少dynamic视角
This leads to a line of studies in sociology to explore how different social relations affect ones' career success~\cite{seibert2001social, adler2002social, shipilov2014network}. 
However, these attempts analyze the problem in a static manner using a snapshot of the social relation, while ignoring the dynamic changes of relations.
This hinders the analysis of the dynamic effects of relations on career evolvement. 
% 3-4 现在很多工作都是statistic-based methods，费劲
Moreover, the current statistic-based methods require significant efforts for analysis. 
They are ill-suited to efficiently explore the academic careers with social relations from overview to details, thus hindering researchers from understanding the findings detected due to large amount of data. 

% 4. Three challenges for developing a visualization system
These obstacles have motivated us to utilize visual analytics to analyze academic career success dynamically and interactively. 
However, developing such a visual analytics system faces three challenges.
% 4-1 model
First, analyzing the effects of multiple factors including social relations are difficult. 
Academic career success can be influenced by historical performances of multiple factors. 
Capturing the dynamic change and analyzing the effects of different factors on career success are difficult. 
The effects of social relations aggravate the complexity of the problem. 
Thus, a sophisticated modeling of the problem is required to distill prototypical patterns of different factors and analyze their affects on academic career success. 
% 4-2 visualization design
Second, depicting the effects of multiple factors on career success is challenging. 
Given a large set of researchers' academic profiles with a long time span, the visual representation of multiple factors' effects requires supporting both lateral comparison of different groups and longitudinal comparison within one group. 
% 4-3 visual analytics system
Third, supporting interactive exploration of the effect of multiple factors on academic career success from overview to detail is non-trivial. 
Apart from the general patterns distilled from the whole data, users also desiderate to explore the academic profiles in different levels of detail (LODs) to compare and reason the result in a more comprehensive approach~\cite{shneiderman2003eyes}. 
An interactive system with additional statistics for further reasoning is thus required. 

% 5-our methods
To address above challenges, we first proposed an enhanced framework based on sequence history analysis (i.e., SHA)~\cite{rossignon2018sequence} to detect the multi-factor effects on the academic career success. 
We then propose novel visual designs to reveal the factor effects along time from different levels of detail (i.e., LODs). 
Particularly, we utilized a \wyf{factor timeline} to compare the effects of factors along time. 
A \wyf{career line} enhanced with multiple factors are designed to show the academic career development in a micro level. 
Based on the framework and visual design, we further propose \textit{\systemname}, an interactive visualization system that assists both \wyf{sociologists and general researchers} in exploring and comparing academic career success with multiple factors at different periods. 
Our contributions are listed as follows: 
\vspace{-0.2cm}
\begin{itemize}
    \item \wyf{We characterize the problem domain of visual analytics of multi-factor effect on career success into three aspects, namely, xxx.} 
    % \item We proposed a novel SHA-based framework that extract career mobility patterns and analyze networking effects on one's career success at different time periods. 
    \vspace{-0.6cm}
    \item We design and develop \textit{\systemname}, an interactive visualization system that enables \wyf{sociologists and general researchers} to identify and explore insightful patterns of academic careers with multiple factors using novel \wyf{matrixline and careerline} designs. 
    \vspace{-0.2cm}
    \item \wyf{We demonstrate the effectiveness and usability of \textit{\systemname} with a real world usage scenario \wyf{and a user study}.} 
\end{itemize}



 


==> sections/01_Introduction_history/01_Introduction_20210324.tex <==
\firstsection{Introduction}
\label{sec:01_Introduction}
\maketitle
% What we sell: 
% (1) For science-of-science, 具体缺点不确定(请Winson补充)。但是看了几篇paper，做的都是整个research领域的一些研究，而并没有“长期追踪”一个领域的一群人（但我不清楚为什么要这么做，只是我们是这么做的）
% (2) For career mobility analysis, 
%    2-1 大部分工作只做clustering，找pattern。
%    2-2 他们不做multi-factor correlation analysis. (尤其是social network这个因素，更复杂)
%    2-3 有个别工作做了social network + career mobility, 但是都是static的

% 所以我们sell:
% 1. multi-factor analysis (+social network)
% 2. from a temporal perspective (因为领域在发展，不同的factor影响也在变)

% 1. concept: career mobility. and its importance
Nowadays, career mobility has been widely studied in both sociology and data science. 
It studies career paths in terms of transitions in job-related attributes such as incomes and positions~\cite{rosenbaum1979tournament}. 
It is essential to understand social mobility at the population level and facilitate career success at the individual level. 
% 
% 2. academic career success
With the increased availability of \wyf{academic profiles} such as researcher careers and their scientific outputs, 
academic careers has become one of the essential topics in career mobility studies. 
It has attracted the attention of both \wyf{sociologists and general researchers} to understand the \wyf{``fundamental drivers of science and improve the scientific enterprise.''}~\cite{fortunato2018science}. 
Sociologists focus on how different factors influence career success, which is a major topic in life-course data analysis. 
General researchers are concerned with how to raise scientific productions and achieve their career success. 
These have brought a heated discussion in the area of Science of science (i.e., SciSci)~\cite{fortunato2018science}.  
Researchers use the academy profiles to understand how different factors that may drive academic career success. 
It can further facilitate decision-making and raise scientific production of the whole research community. 

% 3. 然而现在的工作有缺陷
% 3-1 SciSci - 很多工作（VIS领域的几个paper）：只注重一个角度的分析or只是多角度泛泛而谈。不分析多因素影响career success + 动态分析, based on a specific population
However, most existing works in both SciSci and career mobility are inadequate to understand academic career success. 
Most SciSci works hold a single focus (e.g., collaboration~\cite{li2019early} or gender disparities~\cite{huang2020historical}) to analyze the academic success. 
Hardly have them traced a specific group of researchers longitudinally to compare the multi-factor impact on the career success along time. 
This could be essential to understand the problem from a dynamic perspective and reflect the evolution of a specific field. 
% 3-2 以前的career data analysis虽然是动态的分析，但是缺少network
Career mobility studies have considered the career developments from a temporal perspective. 
Traditional works aim to identify common trajectories as patterns, while hardly analyze the multi-factor impacts on the career success. 
Moreover, social relations (such as collaboration), as one of the complex factors, may also play an important role in achieving career success~\cite{li2019early, shipilov2014network}. 
% The sharing of resources such as knowledge through social relations may also influence the academic career success. 
% 3-3 以前也有工作分析social capital + career mobility, 但是缺少dynamic视角
Although a few studies in sociology explored how social relations affect ones' careers~\cite{seibert2001social, adler2002social, shipilov2014network}, they analyze the problem in a static manner using a snapshot of the social relation.
They ignored the changes of relations along time, which hinders analyzing the dynamic effects of social relations on career evolvement. 
% 3-4 现在很多工作都是statistic-based methods，费劲
Moreover, the current statistic-based methods require significant efforts for analysis. 
They are ill-suited to efficiently explore the academic careers with multiple factors from overview to details with large amount of data. 

% 4. Three challenges for developing a visualization system
These obstacles have motivated us to utilize visual analytics to analyze academic career success dynamically and interactively. 
However, developing such a visual analytics system faces three challenges.
% 4-1 model
First, analyzing the effects of multiple factors including social relations are difficult. 
Academic career success can be influenced by historical performances of multiple factors. 
Capturing the dynamic change and analyzing the effects of different factors on career success are difficult. 
The effects of social relations aggravate the complexity of the problem. 
Thus, a sophisticated modeling of the problem is required to distill prototypical patterns of different factors and analyze their affects on academic career success. 
% 4-2 visualization design
Second, depicting the effects of multiple factors on career success is challenging. 
Given a large set of researchers' academic profiles with a long time span, the visual representation of multiple factors' effects requires supporting both lateral comparison of different groups and longitudinal comparison within one group. 
% 4-3 visual analytics system
Third, supporting interactive exploration of the effect of multiple factors on academic career success from overview to detail is non-trivial. 
Apart from the general patterns distilled from the whole data, users also desiderate to explore the academic profiles in different levels of detail (i.e., LODs) to compare and reason the result in a more comprehensive approach~\cite{shneiderman2003eyes}. 
An interactive system with additional statistics for further reasoning is thus required. 

% 5-our methods
To address above challenges, we first proposed an enhanced framework based on sequence history analysis (i.e., SHA)~\cite{rossignon2018sequence} to detect the multi-factor effects on the academic career success. 
We then propose novel visual designs to reveal the factor effects at different periods. 
Particularly, we utilized a \wyf{factor timeline} to compare the effects of factors along time. 
A \wyf{career line} enhanced with multiple factors are designed to show the academic career development in a micro level. 
Based on the framework and visual design, we further propose \textit{\systemname}, an interactive visualization system that assists both \wyf{sociologists and general researchers} in exploring and comparing academic career success with multiple factors from different levels of detail. 
Our contributions are listed as follows: 
\vspace{-0.2cm}
\begin{itemize}
    \item \wyf{We characterize the problem domain of visual analytics of multi-factor effect on career success into three aspects, namely, xxx.} 
    % \item We proposed a novel SHA-based framework that extract career mobility patterns and analyze networking effects on one's career success at different time periods. 
    \vspace{-0.6cm}
    \item We design and develop \textit{\systemname}, an interactive visualization system that enables \wyf{sociologists and general researchers} to identify and explore insightful patterns of academic careers with multiple factors using novel \wyf{matrixline and careerline} designs. 
    \vspace{-0.2cm}
    \item \wyf{We demonstrate the effectiveness and usability of \textit{\systemname} with a real world usage scenario \wyf{and a user study}.} 
\end{itemize}



 


==> sections/02_RelatedWork_history/02_RelatedWork_20210228.tex <==
\section{Related Work}
\label{sec:02_RelatedWork}

\subsection{Career Mobility Analysis}
\label{sec:02_RelatedWork_CareerDataAnalysis} 
Career mobility studies the trajectories of individuals in terms of transitions in job-related attributes, such as career success (e.g., income and job level) and organizations. 
It has been widely studied in both sociology (in life course studies) and data science (in event sequence analysis) due to its inherent sequence characteristic.

Sociologists focus on a macro-level analysis.
They aims to extract common career patterns to have an overall picture of the whole population. 
Early study conduct cross-sectional analysis over short time periods to study inflow and outflows across different occupations~\cite{rosenbaum1979organizational, hout1983analysing}. 
With the increasing availability of life-course data, longitudinal career analysis become a mainstream~\cite{nagin2016group, liao2020filipino}. 
They use sequence analysis to cluster career paths into different mobility categories based on similarities. 
However, these approaches are semi-automatic which require large efforts for analysis. 
% 
Data mining scientists focus on a micro-level study. 
Prediction on the next career event~\cite{xu2015learning, meng2019hierarchical} and comparison among different individuals~\cite{xu2014modeling} are two types of studies. 
However, such fine-grained analysis lacks a macro summary of career paths, which are essential for understanding human behaviors in sociology. 

Many data visualization studies also incorporate career data as a usage scenario in the event sequence analysis. 
Most works study from a single purpose, including similarity analysis~\cite{janicke2015interactive, du2016eventaction, filipov2019cv3} and visual sequence summarization~\cite{guo2017eventthread, guo2018visual}. 
Filipov \etal~\cite{filipov2019cv3} presented a visualization system to compare multiple resumes that assist company recruiters efficiently find suitable candidates. 
Du \etal~\cite{du2016eventaction} and Jänicke \etal~\cite{janicke2015interactive} developed two systems respectively to recommend similar career paths of students or musicians for a target individual. 
Instead of clustering based on the whole sequence, Eventthread~\cite{guo2017eventthread} and ET2~\cite{guo2018visual} conduct a more fine-grained clustering and summarize academic career paths into multiple latent stages. 

% 
However, above works all assume that career paths are independent from each other, ignoring the effect of networking on career mobility. 
A small set of studies in sociology analyze the impact of social capital (e.g., different social networks) on one's career success~\cite{seibert2001social, ganiron2013social, shipilov2014network}. 
Yet mostly they analyze from a static perspective based on the social network collected at the present time of the survey.
They ignore the dynamics of networking, which would lead to dynamic change of networking impact on career success. 
Several visualization systems also contain social networks in career analysis. 
In the Interactive Chart of Biography~\cite{khulusi2019interactive}, several relations such as institutional and denominational ties are distilled to show the relationships of musicologists. 
Resumevis~\cite{zhang2018resumevis} contains an ego-network based graph that summarizes the career relations (e.g., co-working) of the focused individual. 
Nevertheless, these social networks are regarded as supplementary information to study career mobility. 
They have not correlate the social network with career performance. 
In this work, we propose a new framework to analyze networking effects on career paths dynamically and further provide an interactive visualization system to explore the career mobility more efficiently. 

\subsection{Sequence Analysis}
\label{sec:02_RelatedWork_SequenceAnalysis}
Event sequences are continually studied in the past decades in both sociology and computer science with many research focuses overlapped. 
Based on the survey of Guo \etal~\cite{guo2020survey} and Piccarreta~\cite{piccarreta2019holistic}, sequence analysis in both disciplines can be summarized into three categories, namely, pattern discovery, sequence inference, and sequence modeling. 
Since our focuses are analyzing career mobility patterns and networking effects on career success, we would discuss the most relevant works. 

Sequence clustering is a universal technique to extract common sequential patterns using unsupervised learning. 
Xu \etal~\cite{xu2005survey} summarized different clustering strategies into three categories, namely, proximity-based, feature-based, and model-based. 
Specifically, proximity-based methods use distance matrix to measure the similarity of sequences. 
It is widely adopted in both data science~\cite{xu2005survey} and sociology~\cite{ritschard2018sequence, piccarreta2019holistic}.
Analysts first compute the pairwise dissimilarities between sequences and use clustering approaches to find common sequential patterns. 
The critical step in proximity-based methods is to construct distance matrix. 
A lot of sequence dissimilarity measures are proposed~\cite{studer2016matters, xu2005survey} such as Euclidean distance and Levenshtein distance. 
Besides clustering on the entire sequences, a many methods propose to conduct stage analyze to represent the sequence progression with more details~\cite{guo2017eventthread, guo2018visual}. 
% 
In addition to clustering, sequence inference (also noted as event history analysis in sociology) is another enduring topic. 
This line of works estimate the influence of historical events or trajectories on the upcoming events.  
Graphical models~\cite{stopar2018streamstory, bhattacharjya2020event} and regression analysis~\cite{stopar2018streamstory}. 

In this paper, we adopt the approach from Rossignon \etal~\cite{rossignon2018sequence} which combines sequence clustering with sequence inference to analyze the influence of how individuals' career paths in one's social network would affect his current career success. 


\subsection{Event Sequence Visualization}
\label{sec:02_RelatedWork_EventSequenceVisualization}
A variety of visualization techniques are developed to present event sequence data. 
Guo \etal~\cite{guo2020survey} have proposed a comprehensive survey of event sequence visual analytics approaches. 
Here we mainly summarize the most relevant visualization techniques in career mobility analytics. 

A large amount of designs adopt the horizontal timeline encoding, which is intuitive. 
Based on this encoding, flow-based visualization is a common representation with good scalability to summarize large scale sequence data, including tree-based~\cite{monroe2014interactive, liu2017coreflow} and Sankey-based~\cite{gotz2014decisionflow, wongsuphasawat2012exploring} structures. 
Two strategies are commonly used to reveal sequential patterns with fine granularity. 
One is to use stage analysis to extract latent stages within the whole sequence to show progressions~\cite{guo2017eventthread, guo2018visual}. 
The other is to directly visualize original individual sequences as horizontal lines~\cite{plaisant2003lifelines, di2020sequence}. 
Recent work by Bartolomeo \etal~\cite{di2020sequence} further use layered directed acyclic network together with layout optimization to align specific events among sequences. 
Similar visual representations are adopted in storyline visualization~\cite{tang2018istoryline, tang2020plotthread} with each line represent an actor and the vertical position representing groupings of actors according to different events. 
Another set of works use matrix- or list-based techniques to visualize event sequences which is also scalable~\cite{zhao2015matrixwave, du2016eventaction, wu2017ittvis}. 

However, most of the state-of-the-art focus on pattern extraction and only consider the relative time, which align sequences to the same starting point. 
It cannot be directly used in career mobility and networking analysis, since the absolute time is also of great importance. 
For example, the relations such as collaborations always take over an overlapped time segment, which may affect ones career success in that period. 
Moreover, a single type of visualization granularity (e.g., lines or flows) is inadequate in career mobility analysis. 
It requires the analysis of group patterns, as well as detailed individual inspections together with social relations embedded, which thus calls for novel visual designs. 

% \wyf{\subsection{Dynamic Network Visualization}}

% \wyf{\subsection{Researcher Profile Visualization}}

==> sections/02_RelatedWork_history/02_RelatedWork_20210324.tex <==
\section{Related Work}
\label{sec:02_RelatedWork}

\subsection{Career Mobility Analysis and Visualization}
\label{sec:02_RelatedWork_CareerDataAnalysis} 
% 1. career mobility definition
Career mobility studies the trajectories of individuals in terms of transitions in job-related attributes, such as career success (e.g., income and job level) and organizations. 
It has been widely studied in both sociology (in life course studies) and data science (in event sequence analysis) due to its inherent sequence characteristic.

% 2. Sociologists (group-level) & Data mining scientists (individual-level)
Sociologists focus on a macro-level analysis which aims to extract common career patterns. 
Early studies conduct cross-sectional analysis over short time periods to learn inflow and outflows across different occupations~\cite{rosenbaum1979organizational, hout1983analysing}. 
With the increasing availability of life-course data, longitudinal career analysis become a mainstream~\cite{nagin2016group, liao2020filipino}. 
They use sequence analysis to cluster career paths into different categories based on similarities. 
However, these approaches are semi-automatic and require large efforts for analysis. 
% 
Data mining scientists focus on a micro-level study. 
Prediction on the following career event~\cite{xu2015learning, meng2019hierarchical} and comparison among different individuals~\cite{xu2014modeling} are two major tasks. 
However, such fine-grained analysis lacks a macro summary of careers, which are essential to understand human behaviors in sociology. 

% 3. Visualization field: single focus - network/event summary/similarity
Many visualization studies also incorporate career data as a scenario in the event sequence analysis. 
Most works study based on a single purpose, including similarity analysis~\cite{janicke2015interactive, du2016eventaction, filipov2019cv3} and visual sequence summarization~\cite{guo2017eventthread, guo2018visual}. 
Filipov~\etal~\cite{filipov2019cv3} presented a system to compare multiple resumes that assist recruiters in efficiently finding suitable candidates. 
Du~\etal~\cite{du2016eventaction} and Jänicke~\etal~\cite{janicke2015interactive} developed two systems respectively to recommend similar career paths of students or musicians for a target individual. 
Instead of clustering based on the whole sequence, Eventthread~\cite{guo2017eventthread} and ET2~\cite{guo2018visual} conduct a more fine-grained clustering and summarize academic career paths into latent stages. 

% 4. career mobility + networking
However, most of above works lie in finding common career patterns by either clustering or visual summary. 
Hardly have them considered incorporating multiple factors that may affect career success. 
Moreover, they ignore the effect of networking on careers. 
Several studies in sociology analyze the impact of social networks on one's career success~\cite{seibert2001social, ganiron2013social, shipilov2014network}. 
Yet most of them discuss from a static perspective based on a static social network obtained at a specific timestamp. 
They ignore the dynamics of networking, which would lead to dynamic changes of impact on career success. 
Some visualization systems also contain networking in career analysis. 
In the Interactive Chart of Biography~\cite{khulusi2019interactive}, institutional and denominational ties are distilled to show the relationships of musicologists. 
Resumevis~\cite{zhang2018resumevis} contains an ego-network-based graph that summarizes the co-working relations of the target individual. 
Nevertheless, these social networks are regarded as supplementary information. 
They have not correlate the social network with career success analysis. 
In this work, we propose a new framework and an interactive visualization system to analyze the effect of multiple factors including networking on academic career paths efficiently. 

\subsection{Sequence Analysis}
\label{sec:02_RelatedWork_SequenceAnalysis}
Event sequences are continually studied in the past decades in both sociology and computer science with many research focuses overlapped. 
Based on the survey of Guo~\etal~\cite{guo2020survey} and Piccarreta~\cite{piccarreta2019holistic}, sequence analysis in both disciplines can be summarized into three categories, namely, pattern discovery, sequence inference, and sequence modeling. 
Since our focuses are analyzing multiple factors' impact on career success, we would discuss the most relevant works. 

Sequence clustering is a universal technique to extract common sequential patterns using unsupervised learning. 
Xu~\etal~\cite{xu2005survey} summarized different clustering strategies into three categories, namely, proximity-based, feature-based, and model-based. 
Specifically, proximity-based methods use distance matrix to measure the similarity of sequences. 
It is widely adopted in both data science~\cite{xu2005survey} and sociology~\cite{ritschard2018sequence, piccarreta2019holistic}.
Analysts first define and compute the pairwise dissimilarities between sequences and use clustering approaches to find common sequential patterns. 
The critical step in proximity-based methods is to construct distance matrix. 
A lot of sequence dissimilarity measures are proposed~\cite{studer2016matters, xu2005survey} such as Euclidean distance and Levenshtein distance. 
Besides clustering on the entire sequences, several works propose to use stage analysis to represent the sequence progression with more details~\cite{guo2017eventthread, guo2018visual}. 
% 
In addition to clustering, sequence inference (also noted as event history analysis in sociology) is another enduring topic. 
This line of works estimate the influence of historical events or trajectories on the upcoming events.  
Graphical models~\cite{stopar2018streamstory, bhattacharjya2020event} and regression analysis~\cite{stopar2018streamstory} are widely used. 

We enhance the approach by Rossignon~\etal~\cite{rossignon2018sequence} which combines sequence clustering with sequence inference to analyze the effects of historical records of multiple factors on the present career success. 

\subsection{Event Sequence Visualization}
\label{sec:02_RelatedWork_EventSequenceVisualization}
A variety of visualization techniques are developed to present event sequence data. 
Guo~\etal~\cite{guo2020survey} have proposed a comprehensive survey of event sequence visual analytics approaches. 
Here we mainly summarize the most relevant visualization techniques in career analytics. 

A large amount of designs adopt the intuitive horizontal timeline encoding. 
Flow-based visualization is a common representation with great scalability to summarize large scale sequence data, which includes tree-based~\cite{monroe2014interactive, liu2017coreflow} and Sankey-based~\cite{gotz2014decisionflow, wongsuphasawat2012exploring} structures. 
Two strategies are commonly used to reveal sequential patterns with fine granularity. 
One is to use stage analysis to extract latent stages within the whole sequence to show progressions~\cite{guo2017eventthread, guo2018visual}. 
The other is to directly visualize original individual sequences as horizontal lines~\cite{plaisant2003lifelines, di2020sequence}. 
Recent work by Bartolomeo~\etal~\cite{di2020sequence} further use layered directed acyclic network together with layout optimization to align specific events among sequences. 
Similar visual representations are adopted in storyline visualization~\cite{tang2018istoryline, tang2020plotthread} with each line represent an actor and the vertical position representing groupings of actors according to different events. 
Another set of works use matrix- or list-based techniques to visualize event sequences which are scalable~\cite{zhao2015matrixwave, du2016eventaction, wu2017ittvis}. 

However, most of the state-of-the-art focus on pattern extraction and only consider the relative time, which align sequences to the same starting point. 
It cannot be directly used in academic career success analysis with networking, since the absolute time is also of great importance. 
For example, the relations such as collaborations always take over an overlapped time segment, which may affect ones career success in specific periods. 
Moreover, a single type of visualization granularity (e.g., lines or flows) is inadequate. 
It requires the analysis of group patterns and detailed individual inspections, which thus calls for novel visual designs. 

\subsection{Academic Profile Visualization}
\label{sec:02_RelatedWork_AcademicProfileVisualization} 
The increased availability of academic profile data (e.g., Aminer~\cite{tang2008arnetminer}, Vispubdata~\cite{isenberg2016vispubdata}, and DBLP~\cite{ley2002dblp}) has provided new opportunities to learn the scientific productions from a collective perspective. 
Such multi-dimensional data have attracted visualization researchers for a long time. 
There are three categories according to the major research entities: reseacher-based, paper-based, and hybrid works. 

In researcher-based studies, the collaboration network is a natural type of data to learn ego-network evolution (Egoslider~\cite{wu2015egoslider} and Egolines~\cite{zhao2016egocentric}). 
Fung~\etal designed a tree metaphor to visualize one's publications~\cite{fung2016design}. 
VIS Author Profiles utilize a template-based natural language generation to present a researcher's multiple profiles, such as research topics, major collaborators, and publications. 
% 
For paper-based works, VIStory~\cite{zeng2020vistory}, PivotPaths~\cite{dork2012pivotpaths}, and PaperVis~\cite{chou2011papervis} summarized a group of papers to show the paper collection information from different perspectives such as topics and venues. 
PaperLens~\cite{lee2005understanding} shows the temporal topic trends in conferences. 
% 
Other works go deeper to use novel designs (e.g., linked matrix and flower metaphor) to show scientific impact or influences of different research entities such as authors and conferences~\cite{shin2019influence, wang2018visualizing}. 

However, most of the work focus on the visualization of academic profile data. 
Few have studied the factors that influence researchers' career success, which is an active field in the whole research community (i.e., Science of Science). 
In this work, we use these bibliographic data (including collaboration networks and citations) with academic career data to understand how different factors affect researchers' academic success. 











% \wyf{\subsection{Dynamic Network Visualization}}


==> sections/03_Background_history/03_Background_20210325.tex <==
% Task types: J. Bertin. Semiology of Graphics. University of Wisconsin Press,1983.
% Tasks (questions) in data analysis can be differentiated according to the reading levels: elementary (referring to individual data items), intermediate (referring to groups of data items), and overall (referring to a whole data set).

% primary collaborators
\section{Background and System Overview}
\label{sec:03_Background}
In this section, we introduce the background and concepts of our study, summarize the analytical tasks, and provide a system overview to demonstrate the whole pipeline. 

% 整个过程非常繁琐，需要不断地尝试参数、换方法、定k...; 而且并不能够比较时间线上影响力的变化 -- 专家传统workflow

\subsection{Background and Concepts}
\label{sec:03_Background_Concepts} 
The study of academic career success has been an enduring topic in multiple fields such as SciSci and sequence analysis~\cite{ritschard2018sequence}. 
Learning the dynamic affects of factors on academic career success can benefit both the individual development for the general researchers and the understanding of typical career patterns for sociologists. 


To this end, this work involves the following concepts to characterize the problem of multi-factor effect on academic career success.  
\vspace{-0.2cm}
\begin{itemize}
    \item \textit{Career Success} refers to the outcomes of ones' working experiences~\cite{seibert2001social, arthur2005career}. 
    It can be described by either objective (e.g., job level and income) or subjective measures (e.g., career satisfaction). 
    In the academic careers, \textit{citations} are commonly used as a measure of career success~\cite{fortunato2018science}. 
    \vspace{-0.2cm}
    \item \textit{Career Factors} refer to potential factors that can affect researchers' career success. 
    It includes both individual (e.g., personal abilities) and social factors (e.g., social relations)~\cite{zacher2019academic}. 
    \wyf{In academic careers, due to the data accessibility, we have selected four types of factors that may be related to the career success based on experts' suggestions, namely, job title levels, sectors (i.e., jobs at different fields such as academy and industry), and research domains as individual factors, and academic collaborators' individual factors as social factors. }
    \vspace{-0.2cm}
    \item \wyf{\textit{Factor Categories} are the different groups identified within a factor based on user-specified definitions such as the quantitative ranges of the factors.}
    % based on the sequence clustering results. 
\end{itemize}

\subsection{Data Description}
\label{sec:03_Background_DataDescription} 


\subsection{Task Analysis}
\label{sec:03_Background_TaskAnalysis} 
The diversity of academic careers have attracted people from sociology and general researchers with multiple focuses. 
Sociologists studying career mobility and sequences are interested in the effects of different factors on career success in a dynamic way. 
In addition to individual factors, they are also interested in how the social factors such as social relations affect one's academic career. 
General researchers are also curious about the diverse effects and hope to find role models to follow to reach their career success. 
In this work, we work closely with sociologists in career mobility and sequence analysis to analyze multi-factor effects on academic careers. 
Specifically, we summarize the analytical tasks into two levels as follows. 

The \textbf{inter-factor-level} task provides an overview of how different factors affect career success. 
\begin{enumerate}[leftmargin=*,label={\textbf{T{\arabic*}}}]
    \setlength{\itemsep}{2pt}
    \setlength{\parskip}{2pt}
    \setlength{\parsep}{2pt}
    \vspace{-2mm}
    % High-level对比
    \item \textbf{How do a factor influence the career success over time?} 
    For longitudinal comparison, experts wish to know how a specific factor effects career success over time. 
    This could be related to the development of the specific academic fields. 
    \item \textbf{What do multiple factors differ from affecting the career success?} 
    Given multiple factors, experts wonder the different effects of factors at a specific time as a lateral comparison. 
    This is to find out the dominant factors influencing career success. 
    The comparison of individual and social factors is of great interest. 
\end{enumerate}

The \textbf{intra-factor-level} tasks drive into one specific factor to compare the change of effects of different categories on career success over time. 
\begin{enumerate}[leftmargin=*,label={\textbf{T{\arabic*}}}]
    \setlength{\itemsep}{2pt}
    \setlength{\parskip}{2pt}
    \setlength{\parsep}{2pt}
    \setcounter{enumi}{2}
    \vspace{-2mm}
    % Low-level对比
    \item \textbf{How a category within a factor changes over time to affect the career success?} 
    The impact of a category would change at different periods. 
    It can reflect the change of the roles of this category across time. 
    \item \textbf{How the categories within a factor differ from affecting the career success?} 
    For each factor, different categories may also have different size of impacts. 
    Figuring out those with high impacts can assist in explaining and providing guidelines for the academic career development. 
\end{enumerate}

The \textbf{individual-level} task gives several concrete examples to help understand the factor effects on the career success. 
\begin{enumerate}[leftmargin=*,label={\textbf{T{\arabic*}}}]
    \setlength{\itemsep}{2pt}
    \setlength{\parskip}{2pt}
    \setlength{\parsep}{2pt}
    \setcounter{enumi}{4}
    \vspace{-2mm}
    \item \textbf{How a researcher's career mobility change over time?} 
    Experts wish to distill a representative individual from the data and study the multi-factor effects on career success from a micro perspective.  
    Revealing the career changes of the researcher across the time can help understand the different academic stages he goes over. 
    \item \textbf{How a researcher's different factors reveal over time?} 
    The multi-factor analysis is required to assist in understanding the career mobility and career success. 
\end{enumerate}

\subsection{System Overview}
\label{sec:03_Background_SystemOverview} 
\textit{\systemname} is a web-based application with three modules, namely, a data preprocessing module, a data analysis module, and a data visualization module (Fig.~\ref{fig:system-overview}). 
The data preprocessing module first collects and cleans researcher's career profile and publication data. 
Then it organizes career paths and factors into multiple sequences and stores into the database. 
The data analysis module utilizes an enhanced SHA-based framework to analyze the different factor affects on the career success. 
They form into the backend of the system which is implemented using Python and MongoDB. 
The data visualization module consists of three views to support analysis, which constructs a frontend application using Vue.js~\cite{vue} and D3.js~\cite{d3}. 

\begin{figure} [!htb]
 \centering 
 \includegraphics[width=\linewidth]{figures/system-overview-20210315.png}
 \vspace{-0.4cm}
 \caption{System overview. \textit{\systemname} has three parts: a data preprocessing module, a data analysis module, and a data visualization module.}
 \vspace{-0.4cm}
 \label{fig:system-overview}
\end{figure}



==> sections/04_Algorithm_history/04_Algorithm_20210325.tex <==
\section{Data Analysis}
\label{sec:04_Algorithm}
In this section, we first introduce the data we use and a set of preprocessing approaches. 
Then we describe a SHA-based framework to simultaneous extract career mobility patterns and analyze correlations of historical behaviors of different factors on career success. 

\subsection{Data Description and Preprocessing}
\label{sec:04_Algorithm_DataDescription} 
In this study, we utilize researchers from the visualization community as an example to illustrate academy career analysis. 
We regard those who have published more than two TVCG papers in which the largest time difference is more than five years as potential visualization researchers. 
We manually check the researchers to filter out those from other fields. 
\wyf{The dataset contains xxx researchers.}
The data we use in this work are from multiple sources. 
First, we collect the researchers' career data (including the institutions and titles) from LinkedIn~\cite{linkedin}, researchers' homepages, and department websites. 
Second, we use the latest version of citation network dataset from Aminer~\cite{tang2008arnetminer}, which includes all the publication metadata of a researcher (e.g. authors, year, venue, title, and abstract). 
Third, we collect the number of citations (by year) of each researchers from Google Scholar~\cite{googlescholar} as a measure of career success~\cite{fortunato2018science}. 

\begin{figure} [!htb]
 \centering 
 \includegraphics[width=\linewidth]{figures/data-table-20210319.pdf}
 \vspace{-0.4cm}
 \caption{Events in each sequences.}
%  \vspace{-0.4cm}
 \label{fig:data-table}
\end{figure}

We conducted a set of data cleaning semi-automatically. 
For the career data, we organized each job into an event with a time duration and an institution. 
% We then partitioned the jobs into full-time and part-time and leave with full-time jobs. 
We manually tagged three sectors, namely, academy, industry, and government based on the institutions. 
We also tagged the \wyf{job titles into three levels (i.e., junior, intermediate, and senior)} based on the experts' suggestions and seniority. 
For the citation network data, we distilled the paper venues and classified them into \wyf{fifteen} categories based on~\cite{ccfstandard}. 
\wyf{We also distill the \wyf{collaborators} of a researcher by year as a type of social relations.} 
For the number of citations, we used Quartile~\cite{quartile} to divide each year's citations into four parts of equal size (i.e., four ranks). 
In addition, we separated the \wyf{top 3\% citation researchers} from the top 25\% to emphasize and inspect the pioneers in the visualization field. 

Finally, we constructed the above data into multiple sequences for each researcher (Fig.~\ref{fig:data-table}). 
\textit{Career Sequences} are composed of events defined by both job levels and citation ranks ordered by year. 
\textit{Domain Sequences} consist of a list of paper venue categories with corresponding numbers of papers each year. 
\textit{Sector Sequences} are sequences of sectors by year. 
\textit{Citation Sequences} are sequences of number of citations by year. 
\wyf{We also use the dynamic collaboration networks as a type of researchers' social relation.} 
These sequences along with the collaboration network are then fed into our SHA-based framework. 

\subsection{Sequence History Analysis}
\label{sec:04_Algorithm_SHA} 
We have enhanced the sequence history analysis (i.e., SHA) in sociology~\cite{rossignon2018sequence} to model the multi-factor impacts on academic careers over a long time period. 
The whole framework consists of four components, namely, sequence slicing, sequence clustering, cluster alignment, and multivariable linear regression (Fig.~\ref{fig:framework}). 

\begin{figure*} [!htb]
 \centering 
 \includegraphics[width=\linewidth]{figures/framework-20210319.pdf}
 \vspace{-0.4cm}
 \caption{SHA-based framework. xxx}
 \vspace{-0.2cm}
 \label{fig:framework}
\end{figure*}

\textbf{Sequence Slicing.} 
Traditional SHA-based methods would take the whole sequence as a unit of analysis due to the short time period and small set of events. 
However, it can not be adopted directly in academic career analysis. 
First, the career lengths of researchers are always with great disparity, where diverse career event types could be involved. 
Second, the development of a scientific field could be of a long time span, which could bring impact changes of factors along time. 
Third, when analyzing the effect of previous trajectories of different factors on the upcoming career events, the farther the historical records are, the less relevant of these records to the upcoming career events (time sensitive). 
% may decrease progressively when the historical records are.
Thus, we arrange the each researcher's career-related sequences (Fig.~\ref{fig:framework}-B1) along the absolute time, and slice them into different time windows of a fixed size (i.e., size $w$, Fig.~\ref{fig:framework}-B2). 
We aim to analyze each time window separately to discover the dynamic impact changes of different factors. 
The window size and time steps of the slicing are flexible for users to fine-tune. 

\textbf{Sequence Clustering.} 
For each factor, directly analyzing the historical sequences impact on the upcoming career success would be difficult due to the inherent complexity of sequences. 
A line of works have extracted a set of summary indicators of the historical sequences (e.g., time duration on each event)~\cite{rossignon2018sequence}. 
However, it is be spurious to choose indicators, which may fail to preserve features that depict the sequences themselves. 
One improvement is to identify typical sequences as representative patterns and analyze how different patterns affect career success. 
This keeps the whole sequence characteristics and reduce the computation amount of the raw sequence at the same time. 
To this end, we conducted sequence clustering on different sequences respectively for each time window (Fig.~\ref{fig:framework}-C1). 
For each type of sequence, we use Euclidean distance to obtain the dissimilarity matrix. 
After comparing different clustering algorithms (e.g., k-means, k-medoids, agglomerative, dbscan, optics, and spectural), we finally chose k-means due to its good results and efficiency. 

\textbf{Cluster Alignment.} 
Cluster alignment within each factor across different time window is required to compare the dynamic change of the same type of sequences on career success. 
\wyf{We first summarize and label the sequence within a time window by year by distilling the event with the largest proportion.
We then compare clusters using these cluster labels and regard those with the same labels as the same clusters (Fig.~\ref{fig:framework}-D).}
% 有一个similarity measurement的公式
% 

\textbf{Multivariate Linear Regression.} 
After the alignment, we conducted multivariate linear regression for each time window ($[t, t+w]$) (Fig.~\ref{fig:framework}-E). 
% 1-regression公式
\begin{equation}
    y_{i} = \beta_{0} + \beta_{1}x_{i1} + \beta_{2}x_{i2} + ... + \beta_{n}x_{in} + \varepsilon_{i},  (i=1,...,n)
\end{equation}
We have designed twelve independent variables (i.e., IVs, including individual factors and social factors) and a dependent variable (i.e., DV) based on our experts' suggestions as follows (Fig.~\ref{fig:regression}): 
\vspace{-0.2cm}
\begin{itemize}
    \item \textbf{$IV_{1}-IV_{6}$}. 
    Six categorical variables that are based on the clustering results of three types of sequences (i.e., \textit{Career Sequences}, \textit{Domain Sequences}, and \textit{Sector Sequences}). 
    $IV_{1}-IV_{3}$ are researchers' own historical sequence. 
    $IV_{4}-IV_{6}$ are the top collaborator of the researcher who had co-authored most papers with the target researcher within the time window. 
    Categorical variables with $n$ \wyf{categories} would transformed into $n-1$ dummy variables before the regression. 
    \vspace{-0.2cm}
    
    \item \textbf{$IV_{7}-IV_{12}$}. 
    To better understand how the social factors (e.g., social relations) affect academic careers, we also distill several numerical variables. 
   \wyf{Each variable in $IV_{7}-IV_{9}$ records the number of collaborators in each sequence clusters, which will be transformed into $n$ variables before the regression.}  
    $IV_{10}-IV_{12}$ counts the number of sequence cluster types for each sequence types. 
    \vspace{-0.2cm}
    
    \item \textbf{$DV$}. 
    We aim to analyze the effect of historical factor sequences on the upcoming career success. 
    Thus, our target dependent variable is the number of citations at the following year of the time window. 
    Since the distribution of raw citations each year is with positive skewed distribution, we took the logarithm of the raw citations as the final dependent variable. 
    \vspace{-0.2cm}
\end{itemize}
% 计算每个系数；同时计算R方之差（inter-factor comparison）
% 还有prediction score
\wyf{We also obtained the difference of $R^{2}$ for each IV to evaluate the explanatory power of this IV in the regression model. 
The regression model, the \textit{p-value} and \textit{coefficient} for each independent variable, the difference of $R^{2}$, and the predicted citations of each researchers are recorded and feed into the visualization system for further analysis.}  
% interactively 选参数（window, #clusters） -->更加方便快捷。

\begin{figure} [!htb]
 \centering 
 \includegraphics[width=\linewidth]{figures/regression-20210319.pdf}
 \vspace{-0.4cm}
 \caption{Independent variables and dependent variable in the multivariate linear regression.} 
%  \vspace{-0.4cm}
 \label{fig:regression}
\end{figure}
